Model Validation in Ontology Based Transformations

Model Driven Engineering (MDE) is an emerging approach of software engineering. MDE emphasizes the construction of models from which the implementation should be derived by applying model transformations. The Ontology Definition Meta-model (ODM) has been proposed as a profile for UML models of the Web Ontology Language (OWL). In this context, transformations of UML models can be mapped into ODM/OWL transformations. On the other hand, model validation is a crucial task in model transformation. Meta-modeling permits to give a syntactic structure to source and target models. However, semantic requirements have to be imposed on source and target models. A given transformation will be sound when source and target models fulfill the syntactic and semantic requirements. In this paper, we present an approach for model validation in ODM based transformations. Adopting a logic programming based transformational approach we will show how it is possible to transform and validate models. Properties to be validated range from structural and semantic requirements of models (pre and post conditions) to properties of the transformation (invariants). The approach has been applied to a well-known example of model transformation: the Entity-Relationship (ER) to Relational Model (RM) transformation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{17}
\providecommand{\publicationstatus}{J. Silva and and F. Tiezzi (Eds.): Workshop on Automated\\ 
Specification and Verification of Web Systems (WWV 2012)\\
EPTCS 98, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.98.4}{10.4204/EPTCS.98.4}}
\pdfoutput=1

